A Method for Constraint Inference Using Pose and Wrench Measurements

Many physical tasks such as pulling out a drawer or wiping a table can be modeled with geometric constraints. These geometric constraints are characterized by restrictions on kinematic trajectories and reaction wrenches (forces and moments) of objects under the influence of the constraint. This paper presents a method to infer geometric constraints involving unmodeled objects in human demonstrations using both kinematic and wrench measurements. Our approach takes a recording of a human demonstration and determines what constraints are present, when they occur, and their parameters (e.g. positions). By using both kinematic and wrench information, our methods are able to reliably identify a variety of constraint types, even if the constraints only exist for short durations within the demonstration. We present a systematic approach to fitting arbitrary scleronomic constraint models to kinematic and wrench measurements. Reaction forces are estimated from measurements by removing friction. Position, orientation, force, and moment error metrics are developed to provide systematic comparison between constraint models. By conducting a user study, we show that our methods can reliably identify constraints in realistic situations and confirm the value of including forces and moments in the model regression and selection process.

==> Applications.tex <==
\subsection{Applications}\label{sec:application}
Manipulator interaction with environment constraints is a well-researched area. Applications can largely be attributed to two main areas: planning around and interacting with environment constraints. Sample-based motion planning is a prevalent method that can generate continuous motion that satisfies environment constraints \cite{SurveySample}. Hybrid position-force control is a method that control of applied forces against a constraint and that can compensate for geometric uncertainty of contact with a constraint \cite{Spong}.

\subsubsection{Inferred constraints to hybrid control}
Using the constraint models and framework described this paper, we provide a case study highlighting constraint inference from a demonstration followed by constraint collision avoidance and application of appropriate forces during robot replay.
First, a human demonstrator uses instrumented tongs to draw on a whiteboard (point-on-plane constraint) and draw against a straight-edge (point-on-line constraint). The task of drawing is delicate and requires precise control for successful replay. Too light of contact will not properly replay the drawing and too hard of contact can destroy the marker and cause excess friction.
During constrained interaction, hybrid control allows for force control to be set in particular orientations. The two constraints are recognized from the human demonstration and decomposed into a frame which dictates force control in the direction perpendicular to the board and position control for other non-constrained directions.
The robot replays the demonstration using optimization-based inverse kinematic and path planning (relaxed IK) to generate feasible robot trajectories while avoiding collisions with the recognized constraints. The results are shown in figure [xyz].

\begin{figure}[h]
\centering
\includegraphics[width=2.5in]{./figures/teaserGdrawing.png}
\caption{The inferred geometric constraint from the inferred demonstration enables the robot to robustly interact with the board while replaying the demonstrated trajectory. The forces are applied perpendicular to the board and against the straight edge to maintain contact. Position control is used to move in the end-effector of the robot along the unconstrained degrees of freedom.}
\label{fig:multfits}
\end{figure}

This demonstrates that the constraint inference system described in this paper can be used to leverage existing technologies for interaction with constraints. Integration of these technologies with constraint inference allows a robot agent to replay a complex trajectory from just a single demonstration.


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> front_matter/intro.tex <==
\section{Introduction}
\IEEEPARstart{T}{asks} performed by robots frequently include constraints. While some constraints such as workspace limits may be known beforehand, constrained motion may also occur as part of a robot's trajectory such as when a manipulator is restricted to linear motion when pulling out a drawer.  Control of a robotic manipulator during constraint interaction is made feasible through knowledge of the constraint \cite{Raibert1981}. This paper presents an approach to constraint recognition that leverages measured force, moment, and kinematic data to identify constraints in demonstrations without user input.

In many areas of human-robot interaction, there is a trend to eliminate the need for explicit programming. This principle has led to a class of programming referred to as teaching by demonstration which includes teaching by teleoperation, kinesthetic teaching, and external observation \cite{Argall2009}\cite{PSMG19}. Without explicit programming, these methods allow a user to provide a physical demonstration from which a robot learns a task. Similarly, it would be desirable to avoid explicit programming of constraints. This motivates the need for constraints to be inferred from a demonstration.

Building a constraint inference system is multifaceted. The system must determine the presence of constrained motion in a demonstration. The system must be capable of fitting a constraint model to measurement data. If there are multiple constraint models, the system must be able to differentiate models and select the most appropriate model for a given set of data. To enable constraint recognition without user input, these areas must be addressed.

\begin{figure}[t]
\centering
\includegraphics[width=3.2in]{./figures/teaserChess.png}
\caption{A User demonstrates a chess move by sliding the knight against the chess board. Fitting the \emph{planar-relaxed constraint} using kinematic information is compared against fitting with a combination of pose and wrench measurements. Kinematic-Wrench fitting is able to identify the plane using considerably fewer samples than kinematic fitting.}
\label{fig:teaser}
\end{figure}

Past work has shown that geometric constraint models can be fit from a demonstration containing sufficient kinematic data, however limited attention has been given to the ability to recognize constraints in short demonstrations. As an example, the method described in \cite{armesto} effectively learns a constraint model and develops a policy to act in the null-space of a constraint, which allows mapping of motion across constraints. To accomplish this, the constraint model is trained using 20 seconds of recorded demonstration data. Particularly when a demonstration is performed in a natural way, there is no guarantee a model can be fit with the available demonstration data. Certain applications might require a constraint inference method that minimizes the data required for fitting.

Constrained motion includes reaction forces and moments. Interpreting real world constraint models as scleronomic constraints (i.e. constraints on pose without time dependence) allows formulation of admissible forces and moments via the principle of virtual work. Forces and moments have a duality with kinematic information that can be leveraged to more confidently understand the specifics of a constraint. Kinematic data exposes constraints by demonstrating admissible motion in unconstrained directions and minimal motion against constrained directions. Wrenches provide the opposite set of information. Wrench data is descriptive in constrained directions and minimal in unconstrained directions. Previous work shows that incorporating force and moment information can be used to validate models that are fit using kinematic data \cite{Subramani2018}.

Representations of constraints can be general (i.e. a broad model that fits many types of constrained motion) \cite{Berenson2009}\cite{Li2017} or can be derived from geometric primitives \cite{arodriguez2008}. Replay of human demonstrations involving contact between known polyhedral, cylindrical, and spherical tools and the environment has been explored in detail \cite{Meeussen2008}\cite{Joris1999}. A general model offers flexibility to learn a wider range of constraints without specification of additional models. Primitive models are more easily understood by human compatriots and often more flexible to perturbations in constraint location.

One consequence of using geometric models is that the appropriate model must be selected from a list of candidate models. Commonly in model selection, methods construct a likelihood metric that allows for the selection of the best model. Another method described in \cite{Subramani2018} disambiguates between models by clustering the demonstration for similar fits over a sliding window. While the method is accurate for a small selection of models, it relies on model-specific heuristics to set the clustering metrics and has high computational complexity.

All of these results stem from the ability to locate constrained motion in a robot demonstration. Some methods rely on the demonstration to exclusively contain the constrained motion. Others leverage user input to segment the demonstration into constrained and unconstrained motion. For example, C-Learn by Perez-D'Arpino and Shah \cite{Perez-DArpino2017} uses different grasp approaches and user-identified key-frames to determine standard geometry such as prismatic constraints, posture constraints, and Task Space Regions (TSRs).

Applications for constraint inference in robotics are numerous. As one example, the method described in \cite{Stilman2007} uses task space constraints to sample joint configurations, which allows for redundant manipulators to avoid workspace collisions. More generally, applications of constraint recognition typically revolve around collision avoidance and enabling feasible object interaction though adjusted control.

The contribution of this paper is in presenting a constraint inference approach that uses kinematic and wrench information to fit geometric constraints from a library of models. Specifically, we incorporate reaction forces and moments in an optimization objective to fit constraint models. We describe an approach to resolve reaction wrenches from wrench measurements. We define a general set of position, force, orientation, and moment error metrics that compare between a fit model and measured data. Finally, we demonstrate a method for model selection that combines metrics and penalizes models of different levels of generality. The product of these contributions is a constraint inference method that can fit certain constraint models with much less data compared to kinematic-only fitting and that does not require explicit user input.

==> front_matter/intro_revamped.tex <==
\section{Introduction}
\IEEEPARstart{T}{asks} performed by robots frequently include constraints. For example, constrained motion may occur as part of a robot's trajectory such as when a manipulator is restricted to linear motion when pulling out a drawer.  
Representing physical interactions as constraints provides information about the permissible motion of objects in the environment and the permissible directions that forces and moments may be applied to them. 
This knowledge informs the robot to restrict its joints to permissible configurations so it does not violate this closed kinematic chain (e.g. to plan motion in the constraint \cite{Berenson2009,Stilman2007,Huh2018}) and to apply safe levels of force against the constraint to achieve the appropriate task specific interaction (e.g. through hybrid control \cite{Raibert1981}).


Information about the constraints in the task is useful for programming a robot, but current approaches to determine constraint parameters are not straightforward. 
% If there were an easy source of constraint information, it would be useful for many robotics applications. 
For example, commercial robotic systems provide hybrid control abilities, however the constraints and their geometry must be determined manually. This makes such control difficult to use, limiting the ability of such systems to perform tasks involving constraints.
One solution is to infer constraints from a human demonstration, which eliminates the need for explicit programming \cite{Argall2009,PSMG19}. 
This paper presents an approach to infer constraints in human demonstrations of recorded force, moment, position, and orientation measurements.

\begin{figure}[t]
\centering
\includegraphics[width=3.2in]{./figures/teaser_espresso_demo.pdf}
\caption{Top: Demonstration of an espresso making task using instrumented tongs consisting of sliding an espresso cup, pulling out a drawer, and actuating an espresso lever.  Center: Inferred constraints in task. Our approach infers the samples associated with each constraint (segmentation), the type of constraint (model selection) and model parameters of each constraint (model regression) in the task.}
\label{fig:teaserEspressoTask}
\end{figure}

Building a system to infer constraints from a human demonstration is multifaceted.
The system must determine when the constrained motion occurs in the demonstration.
The system must be capable of robustly fitting constraint models to measurement data.
If there are multiple constraint models, the system must be able to differentiate models and select the most appropriate model.
It must also perform this inference using a natural demonstration of a task (e.g the espresso making task in Fig. \ref{fig:teaserEspressoTask}), which may involve multiple constraint interactions, short constraint interactions, and other physical interactions such as picking up and placing objects.

Past work, summarized below, has shown that geometric constraint models can be fit from a demonstration containing sufficient kinematic data, however limited attention has been given to the ability to recognize constraints in a short demonstration. For example, the method described in \cite{Leopoldo2018} effectively learns a constraint model and develops a policy to act in the null-space of a constraint, which allows mapping of motion across constraints. To accomplish this, the constraint model is trained using 20 seconds of recorded demonstration data. Particularly when a task is performed in a natural way, there is no guarantee a model can be fit with the available duration of demonstration data. Certain applications might require a constraint inference method that minimizes the data required for fitting.

Representations of constraints can be general (i.e. a broad model that fits many types of constrained motion) \cite{Berenson2009,Li2017} or can be derived from geometric primitives \cite{arodriguez2008}. With geometric primitives, replay of human demonstrations involving contact between known polyhedral, cylindrical, and spherical tools and the environment has been explored in detail \cite{Meeussen2008,Joris1999}. A general model offers flexibility to learn a wider range of constraints without specification of additional models, but is difficult to interpret. On the other hand, primitive models are more easily understood by human compatriots. 

One consequence of using geometric primitive models is that the appropriate model must be selected from a list of candidate models. 
A common approach to model selection is to
construct a likelihood metric that allows for the selection of the best model. Another method described in \cite{Subramani2018} disambiguates between models by clustering the demonstration for similar fits over a sliding window. While the method is accurate for a small selection of models, it relies on model-specific heuristics to set the clustering metrics and has high computational complexity.

Many of the existing constraint recognition methods ignore 
%% MG no noun in subject feels awkward
the problem of
%%
determining when constraints occur in a demonstration. Some methods rely on the demonstration to exclusively contain a single constrained motion \cite{Berenson2009,Li2017}. Others leverage user input to segment the demonstration into constrained and unconstrained motion. For example, C-Learn \cite{Perez-DArpino2017} uses different grasp approaches and user-identified key-frames to determine standard geometry such as prismatic constraints, posture constraints, and Task Space Regions (TSRs).

%Interpreting real world constraint models as scleronomic constraints (i.e. constraints on pose without time dependence) allows formulation of admissible forces and moments via the principle of virtual work. 
%Preliminary work shows that incorporating force and moment information can be used to validate models that are fit using only kinematic data \cite{Subramani2018}. 
%% Our method is an extension of that work.
%Our method builds upon that work.

The contribution of this paper is in presenting a constraint inference approach that uses both kinematic and wrench information to infer geometric constraints from a demonstration.
Our approach can take a recording of a human demonstration and determine what constraints are present, when they occur, and their parameters. It can reliably identify and localize a variety of constraint types, even when the constrained interactions are short. We build upon earlier work \cite{Subramani2018},\cite{SubramaniRAL2018} that uses only kinematics to fit constraint models and uses forces and moment information for validation.

In our new method, we incorporate reaction forces and moments in an optimization objective to fit constraint models. We describe an approach to resolve reaction wrenches from wrench measurements which also contain constraint specific friction wrenches. We define a general set of position, force, orientation, and moment error metrics that are used to compare fit models with measured data. 
The product of these contributions is a constraint inference approach that explicitly recognizes the  physical interaction that occurs when interacting with a constraint, where motions and wrenches are related in a manner dictated by the physics of the constrained interaction.  Our approach takes advantage of both wrench and kinematic measurements which enables improved performance over competing kinematic-only approaches. 
We assess our approach with a human subjects study with 9 participants that confirms both the approach's performance as well as the value of including wrench information in the process.


% These physical constraints impose restrictions on the motion of objects in the environment. 
% They permit application of forces and moments (wrenches) against the physical constraint while restricting motion along certain directions. 

% Knowledge of the constraint is imperative for robot interaction. 
% When a robot arm interacts with a constrained object, the end effector may also be restricted by the constraint creating a closed kinematic chain.

% Applications for constraint inference in robotics are numerous. As one example, the method described in \cite{Stilman2007} uses task space constraints to sample joint configurations, which allows for redundant manipulators to avoid workspace collisions. More generally, applications of constraint recognition typically revolve around collision avoidance and enabling feasible object interaction though adjusted control.



% This principle has led to a class of programming referred to as teaching by demonstration which includes teaching by teleoperation, kinesthetic teaching, and external observation \cite{Argall2009}\cite{PSMG19}.

% Inferring the constraint is useful for robot programming. When a robot arm interacts with constrained objects, the end effector may also be restricted by the constraint creating a closed kinematic chain.
% Knowledge of the physical constraint is imperative for robot interaction. 
% The robot can restrict its joints to permissible configurations so it does not violate this closed kinematic chain to plan motion in the constraint \cite{Berenson2009,Stilman2007,Huh2018}. 
% It can also apply safe levels of force against the constraint to achieve the appropriate task specific interaction through hybrid control \cite{Raibert1981}.

%In many areas of human-robot interaction, there is a trend to eliminate the need for explicit programming. This principle has led to a class of programming referred to as teaching by demonstration which includes teaching by teleoperation, kinesthetic teaching, and external observation \cite{Argall2009}\cite{PSMG19}. Without explicit programming, these methods allow a user to provide a physical demonstration from which a robot learns a task. Similarly, it would be desirable to avoid explicit programming of constraints. This motivates the need for constraints to be inferred from a demonstration.

%Building a constraint inference system is multifaceted. 

% Constraint geometry is typically specified manually (e.g. using a teach pendant). 
% Such specification requires an understanding of constraint geometry which novice users may not have. 
% Constraint geometry may also be difficult to determine explicitly. 
% For example, consider the task of wiping an inclined table. 
% Precisely measuring the orientation and position of the planar surface may be difficult.

% A human demonstration can be used to program constraint interactions \cite{Argall2009}\cite{PSMG19}. 


% This suggests that there is a need to use a better input method that facilitate the programming of constraint interactions. 
